Self-supervised Auxiliary Learning with Meta-paths for Heterogeneous Graphs

Graph neural networks have shown superior performance in a wide range of applications providing a powerful representation of graph-structured data. Recent works show that the representation can be further improved by auxiliary tasks. However, the auxiliary tasks for heterogeneous graphs, which contain rich semantic information with various types of nodes and edges, have less explored in the literature. In this paper, to learn graph neural networks on heterogeneous graphs we propose a novel self-supervised auxiliary learning method using meta-paths, which are composite relations of multiple edge types. Our proposed method is learning to learn a primary task by predicting meta-paths as auxiliary tasks. This can be viewed as a type of meta-learning. The proposed method can identify an effective combination of auxiliary tasks and automatically balance them to improve the primary task. Our methods can be applied to any graph neural networks in a plug-in manner without manual labeling or additional data. The experiments demonstrate that the proposed method consistently improves the performance of link prediction and node classification on heterogeneous graphs.

==> Figures_tex/fig_sup.tex <==
\begin{figure}[ht]

\centering
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-3.6cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/gcn-weight-epoch-1-title.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-1.2cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/gcn-weight-epoch-best-title.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    %\hspace{-1cm}
	\includegraphics[height=3.4cm]{Figures/gcn-weight-epoch-100-title.png}
\end{subfigure}

\centering
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-3.6cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/gat-weight-epoch-1.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-1.2cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/gat-weight-epoch-best.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    %\hspace{-1cm}
	\includegraphics[height=3.4cm]{Figures/gat-weight-epoch-100.png}
\end{subfigure}

\centering
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-3.6cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/gin-weight-epoch-1.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-1.2cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/gin-weight-epoch-best.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    %\hspace{-1cm}
	\includegraphics[height=3.4cm]{Figures/gin-weight-epoch-100.png}
\end{subfigure}

\centering
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-3.6cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/sgc-weight-epoch-1.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    \hspace{-1.2cm}
	\includegraphics[trim=0 0 210 0, clip,height=3.4cm]{Figures/sgc-weight-epoch-best.png}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \centering
    %\hspace{-1cm}
	\includegraphics[height=3.4cm]{Figures/sgc-weight-epoch-100.png}
\end{subfigure}
\caption{Weightinf function $\Vc(\cdot)$ learnt by SELAR+Hint on Last-FM on GCN, GAT, GIN and SGC.}
\label{fig:all_weights}
\end{figure}



==> Sections/memo.tex <==
\emph{\textbf{Auxiliary tasks. }}
To design the auxiliary task, we define the self-supervised learning tasks via generating the meta-path labels.
We generate directly multiple meta-path prediction labels by matrix multiplication of adjacency matrices represented each different relation. e.g., "user-item-user", "item-entity-item" and "user-item-entity-item", etc. 
Our auxiliary tasks are the link prediction for generated meta-path labels.
The primary task benefit from auxiliary tasks by predicting meta-paths which can capture diverse semantic information. 
We evaluate the benefits of the self-supervised auxiliary learning by predicting generated meta-path labels.
 Last-FM and Book-Crossing have 60 and 25 entity relations as shown in Table. \ref{tab:node}. We randomly select 5 types of meta-paths which have the path length is less than 4. The selected meta-path types in Last-FM are 'user-musician-user-musician', 'user-musician-artist.origin-musician', 'user-musician-person.or.entity.appearing.in.film-musician', 'user-musician-actor.film-musician' and 'user-musician-musician.instruments.played-musician'.
For instance, 'user-musician-artist.origin-musician' means that it has a meaningful relation among musicians who are the same place of birth. We infer that 'user-musician-musician.instruments.played-musician' is a given user will be interested in artists playing with same instruments .
In Book-Crossing, 'user-book-user', 'book-user-book', 'user-book-user-book', 'book-genre-book' and 'user-item-written.work.literary.series-book-user' are selected. 'book-genre-book' means that books of the same genre are related. A given user who likes a book series has a meaning that he will like some book series. For link prediction, the primary task, which is performed with the auxiliary task predicting meta-paths, is learned by reflecting the meaning of multiple meta-path.


\emph{\textbf{The number of Auxiliary Tasks.}}
We can use various numbers of meta-paths by varying their node and edge compositions for auxiliary tasks. Considering that a meta-path characterizes heterogeneous relations, we hypothesize the number of meta-paths influences the effects to assist the primary task because the the composition of meta-path relates to the difficulty of auxiliary tasks. Table~\ref{tab:abl_length} presents the results of our model for link prediction as the number of meta-paths used for auxiliary tasks increases. For verify the explicit effects of the meta-path number compared to Vanilla, we do not employ hint network. As shown in Table~\ref{tab:abl_length}, using meta-paths consistently improves the link prediction performance as on average 2.2\% and 3.3\% on Last-FM and Book-Crossing datasets for all base GNNs and their number. In particular, employing 3 meta-paths leads to the largest improvement on both datasets. Note that we can get more than 4\% of performance gain with auxiliary tasks of more than 2 meta-paths on Book-Crossing. We conjecture larger that a task that is moderately difficult rather than too easy one helps with generalization performance. With respect to base GNNs, we find that GIN most remarkably benefits from our auxiliary learning with meta-paths. 


% out both explicit weighting function and auxiliary tasks; \textbf{w/o meta-path}, learning a primary task only with the weighting function; \textbf{w/ meta-path}, training with multiple auxiliary tasks; \textbf{Selar}, learning to learn the primary task by auxiliary tasks; \textbf{Selar+Hint}, training with hint network by predicting meta-path as auxiliary tasks;  \\

% \subsection{Ablation Study}
% To further investigate the effects of Selar, we perform ablation study on two main components such as meta-path length and usages of meta cross-validation

% \input{Tables_tex/tab_num_metapath}


%
%\begin{table}[h]
%  \centering
%  \caption{The results of $AUC$ for link prediction}
%  \label{tab:link prediction}
%  \begin{tabular}{c|c|cc|ccc}
%    \toprule
%    & & & & \multicolumn{3}{c}{Ours} \\
%    \hline
%    Dataset & Basemodel & Vanilla & w/o meta-path & w/ meta-path & Selar & Selar+Hint \\
%    \toprule
%    \multirow{4}{*}{Music} & GCN & 0.7898 & 0.785 & 0.8135 & %\textbf{0.8163} & 0.8162 \\
%    & GAT & 0.809 & 0.81 & 0.8184 & 0.8319 & \textbf{0.8349} \\
%    & GIN & 0.7895 & 0.8081 & \textbf{0.8304} & 0.8211 & 0.8255 \\
%    & SGC & 0.7725 & 0.7759 & 0.7801 & 0.7803 & \textbf{0.7857} \\
%    \midrule
%    \multirow{4}{*}{Book} & GCN & 0.6918 & 0.6967 & 0.697 & \textbf{0.7081} & 0.7075 \\
%    & GAT & 0.6704 & 0.6759 & 0.7026 & 0.7136 & \textbf{0.7247} \\
%    & GIN & 0.6782 & 0.6968 & 0.7442 & 0.7554 & \textbf{0.7587} \\
%    & SGC & 0.6781 & 0.6732 & 0.6933 & \textbf{0.707} & 0.7039 \\

%    \toprule
%  \end{tabular}
%\end{table}








%\begin{table}[h]
%  \caption{Raw}
%  \label{sample-table}
%  \centering
%  \begin{tabular}{c|c|cccccc|c}
%    \toprule
%    & & Hint network & Vanilla & w/o meta-path & 1 meta-path & 3 meta-path & 5 meta-path & w/o MW \\
%    \midrule
%    & GCN & w/o & 0.7898 & 0.785 & 0.8071 & 0.825 & 0.8163 & 0.8135\\
%    & & w/ & - & - & 0.8067 & \textbf{0.8293} & 0.8162 & - \\
%    & GAT & w/o & 0.809 & 0.81 & 0.8226 & 0.8342 & 0.8319 & 0.8184 \\
%    & & w/ &- & - & 0.823 & 0.823 & \textbf{0.8349} & -\\
%    Music & & & & &&&&\\
%    & GIN & w/o & 0.7895 & 0.8081 & 0.8205 & 0.8208 & 0.8211 & \textbf{0.8304} \\
%    & & w/ & - &- & 0.8107 & 0.8146 & 0.8255 & - \\
%    & SGC & w/o & 0.7725 & 0.7759 & 0.7819 & 0.7818 & 0.7803 & 0.7801\\
%    & & w/ &- &-& 0.7844 & \textbf{0.791} &0.7857 & -\\
%    \midrule
%    & GCN & w/o & 0.6918 & 0.6967 & 0.7074 & \textbf{0.7156} & 0.7081 & 0.697\\
%    & & w/ & -&-&0.7037&0.7103&0.7075 & -   \\
%    & GAT & w/o & 0.6704 & 0.6759 & 0.6818 & 0.7169 & 0.7136 & 0.7026\\
%    & & w/ & -&-&0.6894 & \textbf{0.7344} & 0.7247&-\\
%    Book & & & & &&&&\\
%    & GIN & w/o &0.6782 & 0.6968 & 0.6944 & 0.7528 & 0.7554 & 0.7442\\
%    & & w/ & -&-&0.6925 & 0.7551 & \textbf{0.7587} & -\\
%    & SGC & w/o &  0.6781 & 0.6732 & 0.6864 & \textbf{0.7159} & 0.707 & 0.6933\\
%    & & w/ & -&-&0.6857 & 0.7128 & 0.7039 & -\\
    
%    \bottomrule
%  \end{tabular}
%\end{table}


% optimizer - Adam
% embedding dimension - 64 for node classifications
% number of layers are two for all models in node classification tasks.
% For each model, hyper parameters such as learning rate and weight decay are tuned for having best performance using validation datasets.
% \begin{table}[h]
%   \centering
%   \caption{$AUC$ of comparable methods with four base GNN models for link prediction}
%   \label{tab:link prediction}
%   \begin{tabular}{c|c|cc|ccc}
%     %\toprule
%     \hline\hline
%     % \multirow{2}*{Dataset}&\multirow{2}*{Base GNNs}&\multirow{2}*{Vanilla}&\multirow{2}*{w/o meta-path} & \multicolumn{3}{c}{Ours (meta-path)} \\
%     \multirow{2}*{Dataset}&\multirow{2}*{Base GNNs}& \multicolumn{2}{c|}{w/o meta-path} & \multicolumn{3}{c}{Ours (meta-path)} \\
%     %\hline
%     & & CE & MWNet & CE & SELAR & SELAR+Hint \\
%     %\toprule
%     \hline
%     \multirow{5}{*}{Last-FM} & GCN & 0.7898 & {0.7850}$^{*}$ & 0.8135 & \textbf{0.8163} & 0.8162 \\
%     & GAT & 0.8090 & 0.8100 & 0.8184 & 0.8319 & \textbf{0.8349} \\
%     & GIN & 0.7895 & 0.8081 & \textbf{0.8304} & 0.8211 & 0.8255 \\
%     & SGC & 0.7725 & 0.7759 & 0.7801 & 0.7803 & \textbf{0.7857} \\
%     \cline{2-7}
%     & Avg. Gain & 0 & +0.0046 & +0.0204 & +0.0222 & \textbf{+0.0253} \\
%     %\midrule
%     \hline
%     \multirow{5}{*}{Book-Crossing} & GCN & 0.6918 & 0.6967 & 0.6970 & \textbf{0.7081} & 0.7075 \\
%     & GAT & 0.6704 & 0.6759 & 0.7026 & 0.7136 & \textbf{0.7247} \\
%     & GIN & 0.6782 & 0.6968 & 0.7442 & 0.7554 & \textbf{0.7587} \\
%     & SGC & 0.6781 & {0.6732}$^{*}$ & 0.6933 & \textbf{0.7070} & 0.7039 \\
%     \cline{2-7}
%     & Avg. Gain & 0 & +0.0061 & +0.0297 & +0.0414 & \textbf{+0.0441}\\
%     %\toprule
%     \hline\hline
%   \end{tabular}
% \end{table}

% In Last-FM datasets, meta cross-validation works well compared to 1-fold for all models in our two frameworks, Selar and Selar with HintNet.
% Also, in node classification tasks, performance of all models enhance when we apply meta data with meta cross-validation methods.


==> Sections/meta-weight-net.tex <==
\textbf{Meta-Weight-Net}~\cite{han2018coteaching} is a meta-learning framework to train neural networks on noisy or skewed datasets.~\jw{For achieving this, Meta-Weight-Net learns an explicit sample-weight function to maximize its performance on an `ideal' test dataset called `meta-dataset', which contains noise-free or balanced data.} 
%Meta-Weight-Net learns an explicit sample-weight function to train a model on a noisy or skewed training dataset to maximize its performance on an `ideal' test dataset called `meta-dataset', which is a noise-free or balanced data. 
For example, assume that the target task is to learn a classifier $f(\xb; \wb)$, which has a good performance on a meta-dataset.
Meta-Weight-Net learns the sample-weight function $\mathcal{V}(\cdot;\Theta)$ parameterized by $\Theta$ so that 
a regular training with the sample-weights can find an optimal classifier $f(\xb;\wb^{\ast})$ for the meta-dataset.
The optimal parameters $\mathbf{w}^{\ast}$ can be  found by minimizing the following loss:  
% Then, given $N$ training samples, the training seeks the optimal model parameters $\mathbf{w}^{\ast}$ minimizing the weighted training loss given as 
\begin{equation}
\label{eq:mw_optimal}
\mathbf{w}^{\ast}(\Theta) = \underset{\mathbf{w}}{\argmin} \ \mathcal{L}^{train}(\mathbf{w};\Theta) \triangleq \frac{1}{N}\sum_{i=1}^{N} \mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\Theta))\mathcal{L}_{i}^{train}(\mathbf{w}),
\end{equation} 
where $\Lc^{train}_i(\wb)  \triangleq \ell(y_i^{(train)}, f(x_i^{(train)};\wb))$ is the training loss for the $i_{th}$ sample, and $\mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\Theta))$ is the learned sample-weight.~\jw{$N$ denotes the training data size.}
% The weight is determined by parameters of weight function $\Theta$ and its input $L_{i}^{train}(\mathbf{w})$, which is $i$-th sample loss on classifier parameter $\mathbf{w}$.
% The optimal parameter of Meta-Weight-Net is obtained by equation:
% \begin{equation}
% \label{eq:mw_optimal}
% % \mathbf{w}^{\ast}(\theta) = \underset{w}{\argmin} \ \mathcal{L}^{train}(\mathbf{w};\theta) \triangleq \frac{1}{N}\sum_{i=1}^{N} \mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\theta)\mathcal{L}_{i}^{train}(\mathbf{w}),
% \mathbf{w}^{\ast}(\Theta) = \underset{\mathbf{w}}{\argmin} \ \mathcal{L}^{train}(\mathbf{w};\Theta) \triangleq \frac{1}{N}\sum_{i=1}^{N} \mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\Theta))\mathcal{L}_{i}^{train}(\mathbf{w}),
% \end{equation} 
% where $N$ is number of train-data samples and $\mathbf{w}^{\ast}$ is the optimal classifier parameter. The hyper-parameter $\Theta$ is determined automatically in a meta-learning way. The optimal parameter $\Theta^{\ast}$ can be obtained by equation:
To optimize the sample-weights, the parameters $\Theta$ is optimized by 
\begin{equation}
\label{eq:mw_theta_optimal}
\Theta^{\ast} = \underset{\Theta}{\argmin} \ \mathcal{L}^{meta}(\mathbf{w}^{\ast}(\Theta)) \triangleq \frac{1}{M}\sum_{i=1}^{M} \mathcal{L}_{i}^{meta}(\mathbf{w}^{\ast}(\Theta)),
\end{equation}
where $M$ is the number of meta-data samples and $\mathcal{L}_{i}^{meta}(\mathbf{w}) = \ell(y_{i}^{(meta)}, f(x_{i}^{(meta)}, \mathbf{w}))$ is the validation loss on meta-data. 
This can be viewed as a form of meta-learning. 
Inspired by this work, we propose a meta-learning framework to learn a model with multiple auxiliary tasks to improve the performance of the primary task.
% We apply this concept to learn adaptively by learning auxiliary tasks. In section 3.2, we will show how we apply Meta-Weight-Net to train GNN task through multi meta-paths prediction tasks. 

==> Tables_tex/tab_CV_IMDB.tex <==
\begin{table}[h]
  \caption{Comparison between 1-fold and 3-fold as meta-data on \textbf{IMDB} datasets \jw{[결과되게 애매한데 뺄까요? 이테이블?]}}
  \label{tab:metacv_node}
  \centering
  \begin{tabular}{c|c|cc|cc}
    \toprule
     & & \multicolumn{2}{c}{SElAR} & \multicolumn{2}{c}{SELAR+Hint}\\
     
     Model &Vanilla &1-fold & 3-fold & 1-fold & 3-fold  \\
    \midrule
     GCN & 0.5809 & 0.5302 & \textbf{0.5994 }& 0.5663 &\textbf{ 0.5847}  \\
     GAT & 0.5587 & 0.6032 & \textbf{0.6126 }& \textbf{0.6017} & 0.6015   \\
     GIN & 0.5965 & \textbf{0.6140} & 0.5994 & \textbf{0.6015} & 0.5726  \\
     SGC & 0.5583 & 0.5829 & \textbf{0.6224 }& 0.5852 & \textbf{0.5906}  \\
    \bottomrule
  \end{tabular}
\end{table}

==> Tables_tex/tab_MP-Rank.tex <==
%\begin{table*}[h]
%\centering
%\caption{Task-specific weights on \textbf{Last-FM} and \textbf{Book-Crossing} datasets}
%\label{tab:node}
%\begin{tabular}{|l|c||l|c|}
%\hline
%\hline
%\textbf{meta-path} & \textbf{Avg. weighted loss} \\
%$user \xrightarrow{t_1} item \xrightarrow{t_2} actor \xrightarrow{item} item$ &  \\
%\hline
%\end{tabular}
%\end{table*}

\setlength{\tabcolsep}{10pt}
\begin{table}[h]
\centering
\caption{The average of the task-specific weighted loss on \textbf{Last-FM} and \textbf{Book-Crossing} datasets.}
\label{tab:MP}
%\footnotesize 
\begin{tabular}{lc|lc}
\toprule
Meta-paths (Last-FM) & Avg. & Meta-paths (Book-Crossing) & Avg. \\
\midrule
user-item-actor-item & \textbf{7.675} & user-item$^{*}$ & \textbf{6.439} \\
user-item$^{*}$ & 7.608 & user-item-literary.series-item-user & 6.217\\
user-item-appearing.in.film-item & 7.372 & item-genre-item & 6.163\\
user-item-instruments-item & 7.049 & user-item-user-item & 6.126\\
user-item-user-item & 6.878 & user-item-user & 6.066\\
user-item-artist.origin-item & 6.727 & item-user-item & 6.025\\
\bottomrule
{\raggedright ${*}$ primary task \par}
\end{tabular}
\end{table}


==> Tables_tex/tab_datasets.tex <==
%\sy{(+++ 아래 테이블 외관 좀 변경했습니다+++)}\hjk{감사합니다. 이쁘네요.}
\begin{table}[ht]
\centering
\caption{Datasets on heterogeneous graphs.}
\footnotesize 
\label{tab:data}
\begin{tabular}{clrrrr}
\toprule
 & Datasets & \# Nodes & \# Edges & \# Edge type & \# Features \\
%  & \textbf{Dataset} & \ \textbf{\# Nodes} & \ \textbf{\# Edges} & \ \textbf{\#Edge Type} & \ \textbf{\# Features}  \\
 \midrule
\multirow{2}{*}{Link prediction} & Last-FM    & 15,084  & 73,382  & 122 & N/A\\
& Book-Crossing  & 110,739 & 442,746 & 52 & N/A  \\
\midrule
\multirow{2}{*}{Node classification} & ACM    & 8,994  & 25,922 & 4 & 1,902   \\
& IMDB  & 12,772  & 37,288 & 4 & 1,256  \\
\bottomrule
\end{tabular}
\end{table}



% \begin{table*}[h]
% \centering
% \caption{Datasets on heterogeneous graphs.}
% \label{tab:node}
% \begin{tabular}{ccccccc}
% \hline
% \textbf{Dataset} & \ \textbf{\# Nodes} & \ \textbf{\# Edges} & \ \textbf{\#Edge Type} & \ \textbf{\# Features}  \\ \hline
% Last-FM    & 15,084  & 42,346  & 60 & N/A\\
% \\[-0.8em]
% Book-Crossing  & 110,739 & 139,746 & 25 & N/A  \\
% \\[-0.8em]
% ACM    & 8,994  & 25,922 & 4 & 1,902   \\
% \\[-0.8em]
% IMDB  & 12,772  & 37,288 & 4 & 1,256  \\
% \end{tabular}
% \end{table*}

% \begin{table*}[h]
% \centering
% \caption{Datasets for link prediction on heterogeneous graphs.}
% \label{tab:edge}
% \begin{tabular}{ccccccc}
% \hline
% \textbf{Dataset} & \ \textbf{\# Users} & \ \textbf{\# Items} & \ \textbf{\# Interactions} & \ \textbf{\# Entity} & \ \textbf{\# Relations} \\ \hline
% Last-FM    & 1,872  & 3,846 & 42,346 & 9,366 & 60 \\
% \\[-0.8em]
% Book-Crossing  & 17,860  & 14,976 & 139,746 & 77,903 & 25 \\
% \end{tabular}
% \end{table*}

% \begin{table*}[h]
% \centering
% \caption{Datasets for node classification on heterogeneous graphs.}
% \label{tab:node}
% \begin{tabular}{ccccccc}
% \hline
% \textbf{Dataset} & \ \textbf{\# Nodes} & \ \textbf{\# Edges} & \ \textbf{\#Edge Type} & \ \textbf{\# Features} & \ \textbf{ Meta-path} \\ \hline
% ACM    & 8,994  & 25,922 & 4 & 1,902  & PAP, PSP  \\
% \\[-0.8em]
% IMDB  & 12,772  & 37,288 & 4 & 1,256  & MAM, MDM\\
% \end{tabular}
% \end{table*}

==> Tables_tex/tab_link_ablation.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table}[h]
  %\centering
  \caption{Link prediction performance ($AUC$-score) of GNNs}
  \footnotesize 
  \label{tab:add_link_prediction}
  \begin{tabular}{c@{ }c|rrr|rrr}
    \toprule
    %\hline
    Dataset & \shortstack{Base\\GNNs}  & Vanilla & \shortstack{Graph-MW\\ w/o mp} & \shortstack{Graph-MW\\ w/ mp} & SELAR &\shortstack{SELAR\\+Hint } &\shortstack{ Regularized\\SELAR+Hint }\\
    %\toprule
    \midrule
    \multirow{5}{*}{Last-FM} 
    & GCN & 0.7963 & 0.7889 & 0.7885 & 0.8296 & & \\
    & GAT & 0.8115 & 0.8115 & 0.8287 & 0.8307 & & \\
    & GIN & 0.8199 & 0.8217 & 0.8234 & 0.8361 & & \\
    & SGC & 0.7703 & 0.7766 & 0.7691 & 0.7827 & & \\
    \cmidrule{2-8}
    & Avg. Gain & - &  &  &  & & \\
    \midrule
    \multirow{5}{*}{\shortstack{Book\\Crossing}} 
    & GCN & 0.7039 & 0.7031 & 0.7110 & 0.7182 & &\\
    & GAT & 0.6891 & 0.6968 & 0.7075 & 0.7345 & &\\
    & GIN & 0.6979 & 0.7210 & 0.7338 & 0.7526 & &\\
    & SGC & 0.6860 & 0.6808 & 0.6792 & 0.6907 & &\\
    \cmidrule{2-8}
    & Avg. Gain & - & & & & & \\
    \toprule
  \end{tabular}
\end{table}

% \setlength{\tabcolsep}{8pt}
% \begin{table}[h]
%   %\centering
%   \caption{Link prediction performance ($AUC$-score) of GNNs}
%   \footnotesize 
%   \label{tab:add_link_prediction}
%   \begin{tabular}{c@{ }c|rrr|rr}
%     \toprule
%     %\hline
%     Dataset & Base GNNs & Vanilla & \shortstack{Graph-MW\\ w/o meta-path} & \shortstack{Graph-MW\\ w/ meta-path} & SELAR  &\shortstack{ Regularized\\SELAR+Hint }\\
%     %\toprule
%     \midrule
%     \multirow{5}{*}{Last-FM} & GCN & 0.7898 & 0.7850 & 0.7861 & 0.8163 & \textbf{0.8206}\\
%     & GAT & 0.8090 & 0.8100 & 0.8244 & 0.8319 & \textbf{0.8349}\\
%     & GIN & 0.7895 & 0.8081 & 0.8204 & 0.8211 & \textbf{0.8262}\\
%     & SGC & 0.7725 & 0.7759 & 0.7400 & 0.7803 & \textbf{0.8029} \\
%     \cmidrule{2-7}
%     & Avg. Gain & - & +0.0046 & +0.0025 & +0.0222 & \\
%     \midrule
%     \multirow{5}{*}{Book-Crossing} & GCN & 0.6918 & 0.6967 & 0.7047 & 0.7081 & \textbf{0.7109}\\
%     & GAT & 0.6704 & 0.6759 & 0.7075 & 0.7136 & \textbf{0.7290}\\
%     & GIN & 0.6782 & 0.6968 & 0.7543 & 0.7554 & \textbf{0.7602}\\
%     & SGC & 0.6781 & 0.6732 & 0.7038 & 0.7070 & \textbf{0.7088}\\
%     \cmidrule{2-7}
%     & Avg. Gain & - & +0.0061 & +0.0380 & +0.0414 & \\
%     \toprule
%   \end{tabular}
% \end{table}


==> Tables_tex/tab_node_ablation.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table}[h]
  \centering
  \caption{Node classification performance ($F1$-score) of GNNs}
  \footnotesize 
  \label{tab:abb_node_classification}
  \begin{tabular}{cc|rr|rrr}
    \toprule
    Dataset & Base GNNs & Vanilla & Graph-MW & SELAR & SELAR+Hint & \shortstack{ Regularized\\SELAR+Hint }\\
    %\hline
    %\toprule
    \midrule
    \multirow{5}{*}{ACM} & GCN & 0.9034 & 0.9061 & 0.9147 & \textbf{0.9160} & 0.9058\\
    & GAT & 0.9179 & 0.9183 & \textbf{0.9198} & 0.9188 & 0.9095\\
    & GIN & 0.9060 & 0.9100 & 0.9076 & 0.9135 & \textbf{0.9191}\\
    & SGC & 0.9138 & 0.9128 & 0.9158 & \textbf{0.9171} & 0.9124\\
    \cmidrule{2-7}
    & Avg. Gain & - & +0.0015 & +0.0030 & \textbf{+0.0060} & \\
    \midrule
    \multirow{5}{*}{IMDB} & GCN & 0.5826 & 0.5812 & 0.6072 & 0.5970 & \textbf{0.6119}\\
    & GAT & 0.5587 & 0.5697 & \textbf{0.6197} & 0.6017 & 0.5942\\
    & GIN & 0.5965 & 0.5972 & \textbf{0.5994} & 0.5974 & 0.5885\\
    & SGC & 0.5675 & 0.6132 & \textbf{0.6147} & 0.5957 & 0.6088\\
    \cmidrule{2-7}
    & Avg. Gain & - & +0.0140 & \textbf{+0.0340} & +0.0217 & \\
    \bottomrule
  \end{tabular}
\end{table}

